SeamlessGAN: Self-Supervised Synthesis of Tileable Texture Maps

We present SeamlessGAN, a method capable of automatically generating tileable texture maps from a single input exemplar. In contrast to most existing methods, focused solely on solving the synthesis problem, our work tackles both problems, synthesis and tileability, simultaneously. Our key idea is to realize that tiling a latent space within a generative network trained using adversarial expansion techniques produces outputs with continuity at the seam intersection that can be then be turned into tileable images by cropping the central area. Since not every value of the latent space is valid to produce high-quality outputs, we leverage the discriminator as a perceptual error metric capable of identifying artifact-free textures during a sampling process. Further, in contrast to previous work on deep texture synthesis, our model is designed and optimized to work with multi-layered texture representations, enabling textures composed of multiple maps such as albedo, normals, etc. We extensively test our design choices for the network architecture, loss function and sampling parameters. We show qualitatively and quantitatively that our approach outperforms previous methods and works for textures of different types.

==> secs_final_revision/methodology.tex <==

\section{Overview}\label{sec:methodology}



\begin{figure*}[h]
	\centering
	\includegraphics[width=.72\textwidth]{figures/diagrams/DiagramTsv2.pdf}
	\caption[width=1.0\textwidth]{\label{fig:overview}{Overview of \textit{SeamlessGAN}. The input texture stack, represented here by albedo and normal maps $\{A_c, N_c\}$ is fed to an encoder $\mathcal{E}$, which transforms it into a latent space $x_0$. We tile this latent space vertically and horizontally, obtaining a a latent field $\mathcal{F}_0$. $\mathcal{F}_0$ is further processed by several residual blocks $\mathcal{R}_i, i \in \{1, l\}$. The resulting latent variables are transformed by two different decoders,  $\mathcal{G}_a$ and $\mathcal{G}_n$, which will output 4 copies of a seamlessly tileable texture $\{\hat{A},\hat{N}\}$. By cropping the center part of this texture, we obtain a single of those copies, with seamless borders, $\{\hat{A_c},\hat{N_c}\}$. Additionally, this texture can be analyzed by a discriminator $\mathcal{D}$ which provides local estimations of the quality of the synthesis. By analyzing vertical and horizontal search areas $s_v, s_h$, it detects artifacts that may arise when tiling the texture, which gives us an estimation of how \textit{tileable} the texture is. This estimation can be then used by a sampling algorithm for generating high-quality tileable textures. }
	}
\end{figure*}


 In this section, we present the main components of our tileable texture synthesis algorithm \textit{SeamlessGAN}. First, we describe the generative learning framework we use for learning to synthesize textures. %As shown in Figure~\ref{fig:overview}, by leveraging properties of deep latent spaces, 
 We then show how to use this framework for generating tileable textures. Finally, we show how our discriminator can be used for detecting artifacts in the synthesized textures. Using this network as a perceptual-aware error metric, we design a sampling algorithm capable of generating artifact-free tileable textures. 
\subsection{Learning to synthesize textures}\label{subsec:learningframework}
The first step in our tileable texture synthesis framework is to train a generative adversarial network that learns to generate new examples of a single sample texture. We show how to train such a framework for generating tuples of albedo and normal maps, but the network can be extended to a different number of texture maps. 
%\begin{figure}[H]
%	\begin{center}
%		\includegraphics[width=.8\columnwidth]{figures/diagrams/trainingframework.pdf}
%	\end{center}
%	\caption{Diagram of our training framework. The generator receives random $k\times k$ texture maps crops and learns to double their spatial dimensions using a weighted combination of perceptual, adversarial and pixel-wise loss functions.}
%	\label{fig:trainingframework}
%\end{figure}
%Our goal is to train a generative model that can synthesize new texture maps from a single example.
 Specifically, our generative model $G$ outputs a pair of albedo $\hat{A}$ and surface normals $\hat{N}$. Instead of following the typical GAN framework, which relies on a randomly sampled input vector, we use crops $A_c, N_c \in I$ of the input textures $I$ as input to our generative model. %Patch-based training like ours have shown success in many computer vision tasks, as in image stylization or classification~\cite{texler2020interactive, chen2020simple}. 
The generative problem is defined as:
\begin{equation}
\hat{A} , \hat{N} = G(A_c, N_c)
\end{equation}
SeamlessGAN builds upon the work of Zhou et al.~\cite{Zhou2018}. We use \textit{adversarial expansion} to train the network to generate new texture samples. 
During training, random crops of $2k \times 2k$ pixels of the input textures are selected, which will form the target $A_t, N_t \in \mathcal{T}$. The crop for both maps in $\mathcal{T}$ is performed over the same pixels of the texture maps, so as to preserve the spatial coherence between them. From that target crop $\mathcal{T}$, a source random crop $S$ is chosen $A_c, N_c \in S$, with a resolution of $k\times k$ pixels. The goal of the generative network will thus be to synthesize $\mathcal{T}$ given $S$. This learning approach is fully self-supervised.%d, as both target and source images are sampled from the input samples. %As in many other texture synthesis algorithms, a dedicated network is trained for each texture. %, which is computationally expensive. 
The generative model is trained alongside a discriminator $\mathcal{D}$, which learns to predict whether its inputs are the target crops $A_t, N_t \in \mathcal{T}$ or the generated samples $\hat{A} , \hat{N} = G(A_c, N_c)$. %This adversarial training framework proved powerful in \cite{Zhou2018}, and our aim is to extend their method to allow for multiple maps. 

\paragraph{Network architecture}
Our neural network is a generative adversarial network, comprised by an encoder-decoder generator with residual connections, and a convolutional discriminator. So as to be able to synthesize textures of multiple different sizes, the network is designed to be fully-convolutional. We follow the architectural design in~\cite{Zhou2018}, with a few variations. First, building on recent advances on style transfer algorithms, we use \textit{Instance normalization}~\cite{ulyanov2016instance} before each PReLU~\cite{he2015delving} non-linearity operation in both networks. This allows to use normalization for training the networks without the typical artifacts caused by Batch Normalization \cite{ChoiStarGAN:Translation, Deschaintre2018Single-imageNetwork, Ulyanov2016InstanceStylization, Nam2018Batch-instanceNetworks}. Second, in order to allow for the synthesis of multiple texture maps at the same time, we propose a simple variation in the generator architecture.

\paragraph{\textbf{Generator}}
 The baseline architecture proposed in~\cite{Zhou2018} is comprised of three main components: An \textit{encoder} $\mathcal{E}$, which entangles the information of the input texture $\mathcal{T}$ into a deep latent space $x_0\gets\mathcal{E}(\mathcal{T})$,  with half the spatial resolution of the input texture. This latent space is then processed by a set of $l$ \textit{residual blocks} $R_i, i \in \{1,l\}$, which learn a compact representation of the input texture $x_i \gets R_{i} (x_{i-1}) + x_{i-1}$. Finally, a decoder $\mathcal{G}$ transforms the output of the last residual block $R_l$ into an output texture $\mathcal{O} \gets \mathcal{G}(x_l)$. By using residual blocks in the latent space, we are able to train models that only use the levels of visual abstraction that are actually required \cite{he2016deep}, while preserving local details~\cite{ronneberger2015u}.% Not using residual connections would force the model to always use high-level features, which may be rich in semantic information but lose local details that are important for representing the optical appearance of the textures~\cite{ronneberger2015u}.
 
 Synthesizing multiple texture maps with a single generative model poses extra challenges. Each map typically represents different properties of the material, such as micro-geometry or color. Those maps are visually different, meaning that learning to synthesize one of them may not help synthesizing the others. This suggests that different generative models could be needed for each map. However, the texture maps must share pixel-wise coherence, which is not achievable if multiple generative models are used. Following previous work on intrinsic image decomposition~\cite{janner2017self, yu2019inverserendernet, Li_2018_CVPR}, we propose the use of a generative model that learns a shared representation of all the texture maps, but has different decoders for each of them. Such an architecture assumes that the texture properties may be encoded by a dense latent space, but the way in which those latent variables are decoded is different for each texture map. 
 
 As such, our proposed generative network encodes an input texture stack into a deep latent space, and different decoders will transform this latent space into texture maps, which all share pixel-wise correspondence. Specifically, we feed the generative network with a tuple of albedo and normal maps $A_c, N_c$. The encoder $\mathcal{E}$ transforms them into a dense representation $x_0\gets\mathcal{E}(A_c, N_c)$, which is then transformed by the residual blocks, obtaining a shared latent space $x_l$. This is then fed to a decoder for the albedo, which outputs $\hat{A} \gets \mathcal{G}_A(x_l)$ and for the normal map $\hat{N} \gets \mathcal{G}_N(x_l)$. %Even though we propose an architecture capable of synthesizing two texture maps (e.g. albedo and normals), this architecture is easily extensible to allow for the synthesis of more maps, by simply adding more decoders. 

\paragraph*{\textbf{Discriminator}}

For the discriminator $\mathcal{D}$, we follow previous work and use a \textit{PatchGAN} architecture \cite{ Isola2017ImagetoImageTW,Ledig2017Photo-realisticNetwork, Zhou2018}, which, instead of providing a single estimation of the probability of the whole image being real, it is able to classify this likelihood for small patches of it. This architecture has several advantages for our problem. First, it is able to provide local assessments on the quality of the synthesized textures, which we exploit for obtaining high-quality textures. Furthermore, its fully-convolutional architecture allows to provide some control on what kind of features are learned. By adding more deep layers to $\mathcal{D}$, the generated textures are typically of a higher semantic quality, but lose details that may be beneficial to preserve. A detailed study on the impact of the depth of $\mathcal{D}$ can be found on~\cite{Zhou2018}.


\subsubsection*{Training procedure}
Instead of learning to synthesize tileable textures, we train the models to synthesize the textures without accounting for tileability, then leverage their latent spaces for obtaining seamless textures. We thus train the networks following a standard GAN learning framework~\cite{Goodfellow2014GenerativeNets}. We iterate between training the discriminator with a real sample texture stack $\mathcal{T}$ and a generated sample $\{\hat{A}, \hat{N}\}$. The adversarial loss function $\mathcal{L}_{adv}$ is extended with three extra loss terms: $\mathcal{L}_1^a$, $\mathcal{L}_1^n$ and $\mathcal{L}_{style}$. The $ \mathcal{L}_1$ losses measure the pixel-wise distance between generated and target albedo ($\mathcal{L}_1^a$) and normals ($\mathcal{L}_1^n$). To compute the $\mathcal{L}_{style}$, we use the deep perceptual loss described in ~\cite{Gatys_2016_CVPR}.
%This loss function was designed for style transfer of artistic and natural images and trained with ImageNet~\cite{Deng2010ImageNet:Database}, whereas in this problem we use it for texture synthesis. This could mean that this kind of perceptual loss function does not work well for measuring the distance between texture maps different to the albedo, (e.g., normal maps), as the pre-trained network has never seen such images. We observe that this is not the case, and that $\mathcal{L}_{style}$ plays an important role in synthesising the texture faithfully. 
We weight the total style loss by weighting different layers in the same way described in \cite{Rodriguez-Pardo2019AutomaticPatterns, Zhou2018,Gatys_2016_CVPR}. Our global loss function is defined as:
\begin{equation}
\mathcal{L} = \lambda_{adv} \mathcal{L}_{adv} + \lambda_{\mathcal{L}_1^a} \mathcal{L}_1^a + \lambda_{\mathcal{L}_1^n} \mathcal{L}_1^n + \lambda_{style} \mathcal{L}_{style} 
\end{equation}

%To maximize the amount of data used for synthesizing the textures, we do not separate any test dataset. 
Instead of using the network trained for the maximum amount of iterations, we perform the synthesis with the network that minimized the non-adversarial part of the loss function during training: $\lambda_{\mathcal{L}_1^a} \mathcal{L}_1^a + \lambda_{\mathcal{L}_1^n} \mathcal{L}_1^n + \lambda_{style} \mathcal{L}_{style}$. This makes the learning setup more robust to the instability that the discriminator may add to the loss function.


\subsection{Latent space tiling for texture tileability}


Previous work~\cite{Fruhstuck2019TileGAN:Texturesb} showed that by spatially concatenating different latent spaces within a StyleGAN~\cite{karras2019style} generator, it is possible to generate textures that contain the visual information of those tiles while seamlessly transitioning between the generated tiles. Inspired by this idea, we spatially repeat (horizontally and vertically) a single latent space $x_i$ within the generative model, obtaining a latent field $\mathcal{F}_i$. As described in Algorithm~\ref{alg:genseamlesstexture}, we then feed $\mathcal{F}_i$ to the rest of the generator, which outputs a texture stack that contains four copies of the same texture, but which seamlessly transitions between them. By cropping the center portion of this texture stack (with an area of $50\%$ of that of the output texture), we obtain a seamlessly tileable texture stack. %As our model is fully-convolutional, the operations described above can be done in any part of the latent space. %, as the model can process inputs of any resolution. 
An important parameter to select is the level $j$ at which to split the generative process. As shown in Figure~\ref{fig:latentfield}, generating the latent field $\mathcal{F}$ by tiling earlier levels of the latent space forces the network to transform $\mathcal{F}$ more times, thus resulting in more seamlessly tileable textures. We confirm the results found by~\cite{Fruhstuck2019TileGAN:Texturesb} and found that splitting at earlier levels of the latent space ($j\in \{ 1, 2\}$) yields the best visual results. The output texture $O$ has a resolution of $4\times4$ the resolution of the input $\mathcal{T}$. Thus, after the cropping operation, the texture has a resolution of $2\times2$ that of $\mathcal{T}$.

\begin{figure}[t!]
	\centering
	\subcaptionbox{$A_c$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/latent space/input}}
	\subcaptionbox{$\hat{A}, l=1$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/latent space/l1}}
	\bigskip
	\subcaptionbox{$\hat{A}, l=3$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/latent space/l3}}
	\subcaptionbox{$\hat{A}, l=5$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/latent space/l5}}
	\caption{Impact of the latent field level $l$ on the quality of the output tileable textures, using the same input $A_c$. Generating the latent field $\mathcal{F}_l$ early layers ($l=1$) generates the best visual results, later layers either create small artifacts ($l=3$) or generate unpleasant textures ($l=5$).   }\label{fig:latentfield}
\end{figure}
\begin{algorithm}
	\caption{Algorithm for obtaining a tileable texture stack, given an input texture $\mathcal{T}$, a latent space level $j$ and a generative network, with an encoder $\mathcal{E}$, residual blocks $R_i, i \in \{1,l\}$ and a decoder $\mathcal{G}$}\label{alg:genseamlesstexture}
	\begin{algorithmic}[1]
		\Procedure{GenerateSeamlessTexture}{$\mathcal{T}, j, \mathcal{E}, R, \mathcal{G}$}
		\State $i\gets0$
		\State$x_i \gets \mathcal{E}(\mathcal{T})$ \Comment{Encode into latent space}
		\State $i \gets i + 1$
		\While{$i < j$} 
			\State$x_{i} \gets R_i(x_{i-1}) + x_{i-1}$ 
			\State $i \gets i + 1$
		\EndWhile
		\State $\mathcal{F}_i \gets Tile(x_i)$
		 \Comment{Horizontal and vertical tiling}
		\While{$i < l$}
			\State$\mathcal{F}_{i} \gets R_i(\mathcal{F}_{i-1}) + \mathcal{F}_{i-1}$ \Comment{Rest of $R_i$}
			\State $i \gets i + 1$
		\EndWhile
		\State $ O \gets \mathcal{G} (\mathcal{F}_l)$ \Comment{Decode latent field}
		\State \Return $CenterCrop(O)$
	\EndProcedure
	\end{algorithmic}
\end{algorithm}




\subsection{Discriminator-guided sampling algorithm}

As described in Section~\ref{subsec:learningframework}, the generative model is trained in an \textit{adversarial expansion} fashion. The network receives small crops of the sample texture and learns to output textures of twice the spatial resolution of those crops. When synthesizing new textures, however, the fully-convolutional network design allows us to generate textures of any resolution. Even though the textures generated by Algorithm~\ref{alg:genseamlesstexture} are seamlessly tileable, the latent space tiling may generate unwanted artifacts that hinder the realism of the textures, by generating repeating patterns. In contrast to the method in~\cite{Fruhstuck2019TileGAN:Texturesb}, where the latent spaces are drawn from random vectors, ours are encoded representations of input texture stacks. As such, the selection of the input that the network receives plays a role on the quality of the output textures. Our goal now is to provide an automatic solution to this problem. %A naive solution could be to generate an arbitrary number of textures and use a manual process to select the textures that are more visually pleasing. However, such a process would be cumbersome and time-consuming. 
So far, we focused on leveraging properties of the generator for synthesizing tileable textures. This model is trained alongside a discriminator, which allows for local estimations of the quality of the generated textures. We argue, following recent work on generative modeling~\cite{schonfeld2020u}, that the discriminator can work as a semantic-aware error metric that can be exploited for detecting artifacts in the generated textures. As discussed in Section~\ref{subsec:learningframework}, the global loss function contains pixel-wise, \textit{style} and adversarial losses. The adversarial loss learns the semantics of the texture, whereas the other components of the loss functions model color distances or repeated pattern activations~\cite{Rodriguez-Pardo2019AutomaticPatterns}. 

\begin{algorithm}[]
	\caption{Algorithm for classifying a generated texture  as tileable or not tileable, given an input texture  $O$, a Discriminator $\mathcal{D}$, a search area $s$, a threshold $\tau$  }\label{alg:istileable}
	\begin{algorithmic}[1]
		\Procedure{IsTileable}{$O,\mathcal{D}, $s$, \tau$}
		\State $Tileable \gets False$
		\State $\mathcal{P} \gets \mathcal{D}(O)$ \Comment{Output of discriminator}
		\State $s_v \gets verticalArea(\mathcal{P})$ \Comment{Vertical search area}
		\State $s_h \gets horizontalArea(\mathcal{P})$ \Comment{Horizontal search area}
		\State $s_d \gets (\mathcal{P} \cap \overline{(s_v \cup	s_h)})$ \Comment{Rest of  $\mathcal{P}$ }
		\State $m_v \gets min(s_v)$ \Comment{Worst prediction in $s_v$}
		\State $m_h \gets min(s_h)$ \Comment{Worst prediction in $s_h$}
		\State $m_d \gets min(s_d)$ \Comment{Worst prediction in $s_d$}
		\If{$m_v \leq m_d \times \tau$ and $m_h \leq m_d\times \tau$ }
		\State $Tileable \gets True$
		\EndIf
		\State \Return $Tileable$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\begin{figure}[]
	\centering
	\subcaptionbox{$\hat{A_1}$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/discriminator/Successful/albedo}}
	\subcaptionbox{$\mathcal{D}(\hat{A_1})$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/discriminator/Successful/disc}}
	\bigskip
	\subcaptionbox{$\hat{A_2}$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/discriminator/Non-Successful/albedo}}
	\subcaptionbox{$\mathcal{D}(\hat{A_2})$}[.24\linewidth][c]{%
		\includegraphics[width=1\linewidth]{figures/results/discriminator/Non-Successful/disc}}
	\caption{Outputs of $\mathcal{D}$ with textures of different qualities. On the left, a generated albedo $\hat{A_1}$ is artifact-free on the search areas, thus the discriminator ($\mathcal{D}(\hat{A_1})$) is fooled to believe $\hat{A_1}$ is real. On its right, a failed generated sample $\hat{A_2}$ cannot fool the discriminator, which finds artifacts $\mathcal{D}(\hat{A_2})$.  }\label{fig:discriminator}
\end{figure}

Empirically, we find that the artifacts caused by the latent space tiling in Algorithm~\ref{alg:genseamlesstexture} appear on vertical and horizontal frames around the center of the textures. This is likely caused by strong discontinuities or gradients on the same areas of the tiled latent spaces, which the rest of the generative network fails to transform into realistic textures. We propose to use the discriminator's predictions on these areas as an measure of how tileable the texture is. A visualization those predictions under artifact-free inputs and textures with artifacts can be seen on Figure~\ref{fig:discriminator}. The difference between the predicted quality of these areas and the rest of the texture will be our loss function that measures how tileable a texture is. Note that this loss function is learned specifically for each texture. %Besides, the number of layers in the discriminator defines its effective receptive field and, as such, deeper discriminators may look for more semantic patterns but fail to identify smaller artifacts. 
Specifically, as described in Algorithm~\ref{alg:istileable}, we identify whether or not a generated texture $O$ is tileable by looking for artifacts in a vertical and horizontal search area $s$ on the texture, by comparing the predictions $\mathcal{P}$ of $\mathcal{D}$ in $s \in \mathcal{P}$ with the rest of the image $s_d = \mathcal{P} \cap \overline{s}$. As $\mathcal{D}$ outputs $0$ when it believes a patch to be synthetic, we look for artifacts in the predictions by looking for the minimum predicted values on the search areas $s$ and $s_d$. If the minimum value in the vertical and horizontal search areas $s_v, s_h \in s$ are close (measured by $\tau$) to the minimum value in $s_d$, the texture has no artifacts on $s$ and, as such, it is tileable. %The goal of this algorithm is to find tileable textures, not to evaluate the quality of the generated textures and, as such, we do not put any fixed threshold on the predictions of $\mathcal{D}$. 

\begin{algorithm}[t]
	\caption{Sampling algorithm for generating a set $Samples$ of $n$ textures, crop sizes in the range of $c_{max}$ and $c_{min}$, an input $\mathcal{T}$ and $m$ random crops for each crop size.}\label{alg:samplingAlgorithm}
	\begin{algorithmic}[1]
		\Procedure{SampleTextures}{$n,c_{max}, c_{min}, \mathcal{T}, m$}
		\State $c \gets c_{max}$ \Comment{We start at the largest size}
		\State $Samples \gets \{\}$ \Comment{Empty list by default}
		\While{$length(Samples) < n$ or $c\geq c_{min}$}
		\State $i \gets 0$ \Comment{Sample $m$ crops by crop size}
		\While{$i<m$}
		\State $C \gets RandomCrop(\mathcal{T}, c)$
		\State $O \gets GenerateSeamlessTexture(C)$
		\If{$IsTileable(O)$}
		\State $Samples \gets Samples \cup O$ 
		\State $ i \gets i + 1 $ 
		\EndIf
		\EndWhile 
		\State $ c \gets c - 1 $ \Comment{Look for smaller samples}
		\EndWhile
		\State \Return $Samples$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

We propose a discriminator-guided sampling algorithm capable of automatically generating multiple seamlessly tileable textures of different sizes. A main advantage of fully-convolutional generators is that they can generate textures of large sizes, which will organically create less repeating artifacts, as larger textures need to be repeated less times. Consequently, our sampling algorithm will look for tileable textures by randomly cropping the original sample in decreasing sizes. There are two main challenges when finding tileable textures: the size of the input texture has to be adequate so that it models the distribution of the repeating patterns it contains; and the input tile itself must not create strong artifacts when tiling the latent spaces of the generator. Some methods~\cite{lettry2017repeated,Rodriguez-Pardo2019AutomaticPatterns} can estimate the repeating pattern size, but they are limited to regular patterns, which are not common in real-world textures. Consequently, we will sample multiple crop sizes in a decreasing fashion, whilst sampling multiple candidate crops for each crop size. This sampling procedure is described in Algorithm~\ref{alg:samplingAlgorithm}. %We generate random crops of $\mathcal{T}$ of size $c$ by sampling a uniform distribution. 
%We omitted the hyper-parameters for generating seamless textures and classifying them as tileable for simplification. 
This sampling algorithm is designed for square input textures, but it is easily extensible to rectangular shapes.%, as they are also suitable for this fully-convolutional network model. 







